Forward simulation of coherent beams on grating structures for coherent scatterometry

Modelling the scattering of focused, coherent light by nano-scale structures is oftentimes used to reconstruct or infer geometrical or material properties of structures under investigation in optical scatterometry. This comprises both periodic and aperiodic nano-structures. Coherent Fourier scatterometry with focused light exploits the diffraction pattern formed by the nano-structures in Fourier plane. While the scattering of a focused beam by a spatially isolated scatterer is a standard modelling task for state-of-the art electromagnetic solvers based, e.g., on the finite element method, the case of periodically structured samples is more involved. In particular when the focused light covers several grating periods of as it is commonly the case. We will present a coherent illumination model for scattering of focused beams such as Gaussian -- and Bessel -- beams by periodic structures such as line gratings. The model allows to take into account optical wavefront aberrations in optical systems used for both, the illumination and detection of the scattered fields. We compare the model with strategies implemented on large-scale super-cells and inverse Floquet-transform strategies to superimpose both near- and far- fields coherently.

==> figure_6.tex <==

\begin{figure} [ht]
   \begin{center}
   \begin{tabular}{c|c|c|c} %% tabular useful for creating an array of images 
   \includegraphics[height=3cm,trim=0 0 2cm 0]{coherent_pupil_image_unstructured_psi=0.0_11260_32_32.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_32_64.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_32_128.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_32_256.png} \\ 
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_64_32.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_64_64.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_64_128.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_64_256.png} \\ 
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_128_32.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_128_64.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_128_128.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_128_256.png} \\
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_256_32.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_256_64.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_256_128.png} &
   \includegraphics[height=3cm]{coherent_pupil_image_unstructured_psi=0.0_11260_256_256.png}
   \end{tabular}
   \end{center}
   \caption[illuminationSampling] 
%>>>> use \label inside caption to get Fig. number with \ref{}
   { \label{fig:pupil_sampling} \textit{Top:}
Location of the pre-calculated illumination points in the pupil for two different dimensions of the offline database. Points outside the collection NA (red circle) are considered as well due to their Bloch families. 
\textit{Bottom:}
Pupil images for fine illumination pupil and the output sampling. Interpolation artifacts are due to the nearest neighbor interpolation. 
}
\end{figure} 
